DetCo: Unsupervised Contrastive Learning for Object Detection

Unsupervised contrastive learning achieves great success in learning image representations with CNN. Unlike most recent methods that focused on improving accuracy of image classification, we present a novel contrastive learning approach, named DetCo, which fully explores the contrasts between global image and local image patches to learn discriminative representations for object detection. DetCo has several appealing benefits. (1) It is carefully designed by investigating the weaknesses of current self-supervised methods, which discard important representations for object detection. (2) DetCo builds hierarchical intermediate contrastive losses between global image and local patches to improve object detection, while maintaining global representations for image recognition. Theoretical analysis shows that the local patches actually remove the contextual information of an image, improving the lower bound of mutual information for better contrastive learning. (3) Extensive experiments on PASCAL VOC, COCO and Cityscapes demonstrate that DetCo not only outperforms state-of-the-art methods on object detection, but also on segmentation, pose estimation, and 3D shape prediction, while it is still competitive on image classification. For example, on PASCAL VOC, DetCo-100ep achieves 57.4 mAP, which is on par with the result of MoCov2-800ep. Moreover, DetCo consistently outperforms supervised method by 1.6/1.2/1.0 AP on Mask RCNN-C4/FPN/RetinaNet with 1x schedule. Code will be released at \href{https://github.com/xieenze/DetCo}{\color{blue}{\tt github.com/xieenze/DetCo}}.

==> LaTeX/tables/ablation_1.tex <==
\begin{table}[]
\centering
\scalebox{0.95}{
\begin{tabular}{c|c|c|l l|l}
% \hline
 & +MLS & +GLC & Top1 & Top5 & mAP \\ \shline
(a) & $\times$ & $\times$ & 64.3 & 85.6 & 56.3 \\ \shline
(b) & \checkmark & $\times$ & 63.2~$\red{\pmb{\downarrow}}$ & 84.9~$\red{\pmb{\downarrow}}$ & 57.0~$\green{\pmb{\uparrow}}$ \\ \hline
(c) & $\times$ &  \checkmark & 67.1~$\green{\pmb{\uparrow}}$ & 87.5~$\green{\pmb{\uparrow}}$ & 56.8~$\green{\pmb{\uparrow}}$ \\ \hline
(d) & \checkmark & \checkmark & 66.6~$\green{\pmb{\uparrow}}$ & 87.2~$\green{\pmb{\uparrow}}$ & 57.4~$\green{\pmb{\uparrow}}$ \\ 
\end{tabular}}
\caption{\textbf{Ablation:~multi-level supervision~(MLS) and global and local contrastive learning~(GLC)}. The results are evaluated on ImageNet linear classification and PASCAL VOC07+12 detection.}
\label{tab:ab1}
% \vspace{-3mm}
\end{table}

==> LaTeX/tables/ablation_1_new.tex <==
% \begin{table}[h]
% \centering
% \scalebox{0.7}{
\begin{tabular}{c|c|c|l l|l}
% \hline
 & +HIC & +CGLC & Top1 & Top5 & mAP \\ \shline
(a) & $\times$ & $\times$ & 64.3 & 85.6 & 56.3 \\ \shline
(b) & \checkmark & $\times$ & 63.2~$\red{\pmb{\downarrow}}$ & 84.9~$\red{\pmb{\downarrow}}$ & 57.0~$\green{\pmb{\uparrow}}$ \\ \hline
(c) & $\times$ &  \checkmark & 67.1~$\green{\pmb{\uparrow}}$ & 87.5~$\green{\pmb{\uparrow}}$ & 56.8~$\green{\pmb{\uparrow}}$ \\ \hline
(d) & \checkmark & \checkmark & 66.6~$\green{\pmb{\uparrow}}$ & 87.2~$\green{\pmb{\uparrow}}$ & 57.4~$\green{\pmb{\uparrow}}$ \\ 
\end{tabular}
% \caption{
% }
% \label{tab:ab1_new}
% \vspace{-3mm}
% \end{table}

==> LaTeX/tables/ablation_2.tex <==
\begin{table}[]
\centering
\scalebox{0.9}{
\begin{tabular}{c|c|c|l l l l}

    & +MLS & +GLC & Res2 & Res3 & Res4 & Res5 \\ \shline
(a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1 \\ \shline
(b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$ \\ \hline
(c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \hline
(d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$ \\ 
\end{tabular}
}
\caption{\textbf{Ablation:~multi-level supervision~(MLS) and global and local contrastive learning~(GLC)}. Accuracy of feature in different stages are evaluated by PASCAL VOC07 SVM classification.
}
\label{tab:ab2}
% \vspace{-5mm}
\end{table}

==> LaTeX/tables/ablation_2_new.tex <==
% \begin{table}[h]
% \centering
% \scalebox{0.65}{
\begin{tabular}{c|c|c|l l l l}

    & +HIC & +CGLC & Res2 & Res3 & Res4 & Res5 \\ \shline
(a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1 \\ \shline
(b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$ \\ \hline
(c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \hline
(d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$ \\ 
\end{tabular}
% }
% \caption{}
% \label{tab:ab2_new}
% \vspace{-5mm}
% \end{table}

==> LaTeX/tables/ablation_3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\scalebox{0.85}{
\begin{tabular}{l|l|ccc}
    & weight                          & AP   & AP$_{50}$ & AP$_{75}$ \\ \shline
(a) & (0,0,0,1) & 56.3 & 81.8 & 62.1 \\
(b) & (1,1,1,1)+Norm                  & 55.1 & 80.4 & 60.4 \\
(c) & (1,1,1,1)                       & 55.8 & 81.6 & 62.2 \\
(d) & (0.1,0.4,0.7,1)+Norm            & 56.5 & 82.2 & 62.7 \\
(e) & (0.1,0.4,0.7,1)                 & 57.0 & 82.2 & 63.1
\end{tabular}}
\caption{Ablation study of intermediate loss weight, under 100 epoch pre-training. ``Norm'' means normalized the loss weights, making the sum of weights equals 1.0.}
\label{tab:ab3}
\end{table}

==> LaTeX/tables/ablation_4.tex <==
\begin{table}[]
\centering
\scalebox{1.0}{
\begin{tabular}{l|c|ccc}
    & share queue & AP   & AP$_{50}$ & AP$_{75}$ \\ \shline
(a) & \checkmark           & 56.2 & 81.8 & 62.3 \\
(b) & $\times$           & 57.0 & 82.2 & 63.1
\end{tabular}}
\caption{Ablation study of share or not share queue, under 100 epoch pre-training.}
\label{tab:ab4}
\end{table}

==> LaTeX/tables/ablation_5.tex <==
\begin{table}[]
\centering
\scalebox{1.0}{
\begin{tabular}{l|c|c|c|c}
    & $+\mathcal{L}_{g \leftrightarrow g}$ & $+\mathcal{L}_{g \leftrightarrow l}$ & $+\mathcal{L}_{l \leftrightarrow l}$ & AP   \\ \shline
(a) & \checkmark    & $\times$    & $\times$    & 56.0 \\
(b) & \checkmark    & \checkmark    & $\times$    & 56.2 \\
(c) & \checkmark    & \checkmark    & \checkmark    & 56.5
\end{tabular}}
\caption{Ablation study of cross contrastive loss, under 50 epoch pre-training.}
\label{tab:ab5}
\end{table}

==> LaTeX/tables/ablation_both_new.tex <==

\begin{tabular}{p{12pt}<{\centering}|p{20pt}<{\centering}|p{27pt}<{\centering}|p{20pt}<{\centering} p{20pt}<{\centering}|p{20pt}<{\centering} p{5pt}<{\centering} p{12pt}<{\centering}|p{20pt}<{\centering}|p{27pt}<{\centering}|p{20pt}<{\raggedright}p{20pt}<{\raggedright}p{20pt}<{\raggedright}p{20pt}<{\raggedright}}
% \hline
 & +HIC & +CGLC & Top1 & Top5 & mAP & & & +HIC & +CGLC & Res2 & Res3 & Res4 & Res5 \\ \cline{1-6}\cline{8-14}
 
\rule{0pt}{10pt}(a) & $\times$ & $\times$ & 64.3 & 85.6 & 56.3 & & (a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1\\ \cline{1-6}\cline{8-14}

\rule{0pt}{10pt}(b) & \checkmark & $\times$ & 63.2~$\red{\pmb{\downarrow}}$ & 84.9~$\red{\pmb{\downarrow}}$ & 57.0~$\green{\pmb{\uparrow}}$ & & (b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$\\ \cline{1-6}\cline{8-14}

\rule{0pt}{10pt}(c) & $\times$ &  \checkmark & 67.1~$\green{\pmb{\uparrow}}$ & 87.5~$\green{\pmb{\uparrow}}$ & 56.8~$\green{\pmb{\uparrow}}$ & & 
(c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \cline{1-6}\cline{8-14}

\rule{0pt}{10pt}(d) & \checkmark & \checkmark & 66.6~$\green{\pmb{\uparrow}}$ & 87.2~$\green{\pmb{\uparrow}}$ & 57.4~$\green{\pmb{\uparrow}}$  & &
(d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$\\ 
\end{tabular}


% \begin{tabular}{c|c|c|l l l l}

%     & +HIC & +CGLC & Res2 & Res3 & Res4 & Res5 \\ \shline
% (a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1 \\ \shline
% (b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$ \\ \hline
% (c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \hline
% (d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$ \\ 
% \end{tabular}
% }
% \caption{}
% \label{tab:ab2_new}
% \vspace{-5mm}
% \end{table}

==> LaTeX/tables/algorithm1.tex <==

%##################################################################################################
\begin{algorithm}[t]
\caption{Pseudocode of Intermediate Contrastive Loss.}
\label{alg:detco}
\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{2-5}: 4 different stages of backone, termed res2, res3, res4, res5.
%\vspace{-1.em}
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}

\begin{lstlisting}[language=python]
# net_q: encoder for query
# net_q = {backbone_q, head_q_list=[head 2-5]},  

# net_k: same structure as net_q, encoder  for key
# queue_list: a list of queues 2-5 of K keys (CxK)
# m: momentum
# t: temperature
# x: input image
# w: loss weight for 2-5
# loss_nce: contrastive loss

net_q.params = net_k.params  # initialize
x_q = aug(x)  # a randomly augmented version
x_k = aug(x)  # another randomly augmented version

list_q = backbone_q.forward(x_q)  # list of queries
list_k = backbone_k.forward(x_k)  # list of keys

total_loss = 0 # weight-sum of loss from 4 stages
for i in range(4): # loop through 4 stages
    # feature, queue and weight of current stage
    q = list_q[i] # queries: NxC
    k = list_k[i] # keys: NxC
    queue = queue_list[i] # dictionary of K keys (CxK)
    weight = w[i]
    
    # forward mlp head
    q = head_q_list[i].forward(q)
    k = head_k_list[i].forward(k).detach()
    
    # calculate loss
    loss = loss_nce(q, k, queue, t)
    total_loss = total_loss+loss*weight
    
    # update the queue
    dequeue_and_enqueue(queue, k) 

# SGD update: query network
total_loss.backward()
update(net_q.params)

# momentum update: key network
net_k.params = m*net_k.params+(1-m)*net_q.params


\end{lstlisting}
\end{algorithm}
%##################################################################################################

==> LaTeX/tables/cls_det_tradeoff.tex <==
\begin{table}[]
% \centering
\hspace{-2mm}
\scalebox{0.75}{
\begin{tabular}{l|c|cc|c|c}
% \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{Place} & \multicolumn{2}{c|}{ImageNet Cls.}                      & COCO Det. & Cityscapes Seg. \\ \cline{3-6} 
\multicolumn{1}{c|}{}                        &                        & \multicolumn{1}{l}{Top-1} & \multicolumn{1}{l|}{Top-5} & mAP        & mIoU            \\ \shline
MoCo v1\cite{moco}    & CVPR'20 & 60.6 & -    & 38.5 & 75.3 \\ %\hline
MoCo v2\cite{mocov2}    & Arxiv   & 67.5 & -    & 38.9 & 75.7 \\ %\hline
InstLoc\cite{instloc}    & CVPR'21 & 61.7 & -    & 39.8 & -    \\ %\hline
DenseCL\cite{densecl}    & CVPR'21 & 63.6 & 85.8 & 39.3 & 75.7 \\ %\hline
PatchReID\cite{dupr} & Arxiv   & 63.8 & 85.6    & 39.6 & \textbf{76.6} \\ \hline
DetCo      & -       & \textbf{68.6} & \textbf{88.5} & \textbf{39.8} & 76.5 \\ %\hline
\end{tabular}}
\vspace{2mm}
\caption{\textbf{Classification and Detection trade-off for recent detection-friendly self-supervised methods.} 
Compared with concurrent InstLoc\cite{instloc}, DenseCL\cite{densecl} and PatchReID\cite{dupr}, DetCo is significantly better by 6.9\%, 5.0\% and 4.8\% on ImageNet classification. Moreover, DetCo is also on par with these methods on dense prediction tasks, achieving best trade-off.
}
\label{tab:trade}
\vspace{-5mm}
\end{table}

==> LaTeX/tables/sparsercnn.tex <==
\begin{table}[]
\centering
\scalebox{0.9}{
\begin{tabular}{l|l|l|l|l|l|l}
% \hline
          & AP   & AP$_{50}$ & AP$_{75}$ & AP$_{s}$ & AP$_{m}$  & AP$_{l}$  \\ \shline
Supervised   & 45.0 & 64.1 & 49.0 & 27.7 & 47.5 & 59.6 \\ \hline
DetCo & \bf{46.5} & \bf{65.7} & \bf{50.8} & \bf{30.8} & \bf{49.5} & \bf{59.7} \\ 
\end{tabular}}
\caption{\textbf{DetCo \vs Supervised pre-train} on Sparse R-CNN. DetCo largely improves 1.5 mAP and 3.1 AP$_s$.}
\label{tab:sparsercnn}
\end{table}

==> LaTeX/tables/table_c4_fpn_12k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|l l l |l l l |l l l |l l l}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-C4 COCO 12k} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 12k} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &7.9 &16.4 &6.9 &7.6 &14.8 &7.2 &10.7 &20.7 &9.9 &10.3 &19.3 &9.6 \\
Supervised  &27.1 &46.8 &27.6 &24.7 &43.6 &25.3 &28.4 &48.3 &29.5 &26.4 &45.2 &25.7 \\ \hline
InsDis\cite{wu2018unsupervised} &25.8\rbf{-1.3} &43.2\rbf{-3.6} &27.0\rbf{-0.6} &23.7\rbf{-1.0} & 40.4\rbf{-3.2} & 24.5\rbf{-0.8} & 24.2\rbf{-4.2} &41.5\rbf{-6.8} &25.1\rbf{-4.4}&22.8\rbf{-3.6}&38.9\rbf{-6.3}&23.7\rbf{-2.0} \\ 
PIRL\cite{pirl} & 25.5\rbf{-1.6} & 42.6\rbf{-4.2} & 26.8\rbf{-0.8} & 23.2\rbf{-1.5} & 39.9\rbf{-3.7} & 23.9\rbf{-1.4} & 23.7\rbf{-4.7}& 40.4\rbf{-7.9}& 24.4\rbf{-5.1}& 22.1\rbf{-4.3}& 37.9\rbf{-7.3}& 22.7\rbf{-3.0} \\ 
SwAV\cite{swav} &16.5\rbf{-10.6} &35.2\rbf{-11.6} &13.5\rbf{-14.1} &16.1\rbf{-8.6} &32.0\rbf{-11.6} &14.6\rbf{-10.7} &25.5\rbf{-2.9} &46.2\rbf{-2.1} &25.4\rbf{-4.1} &24.8\rbf{-1.6} &43.5\rbf{-1.7} &25.3\rbf{-0.4} \\ 
MoCo\cite{moco} &26.9\rbf{-0.2} &44.5\rbf{-2.3} & 28.2\gbf{+0.6} &24.6\rbf{-0.1} &41.8\rbf{-1.8} &25.6\gbf{+0.3} &25.6\rbf{-2.8} &43.4\rbf{-4.9} &26.6\rbf{-2.9} &23.9\rbf{-2.5} &40.8\rbf{-4.4} &24.8\rbf{-0.9} \\ 
MoCov2\cite{mocov2} &27.6\gbf{+0.5} &45.3\rbf{-1.5} & 28.9\gbf{+1.3} &25.1\gbf{+0.4} &42.6\rbf{-1.0} &26.3\gbf{+1.0} &26.6\rbf{-1.8} &44.9\rbf{-3.4} &27.7\rbf{-1.8} &24.8\rbf{-1.6} &42.1\rbf{-3.1} &25.7\rbf{0.0} \\ \hline
% DetCo &\bf{29.3}\gbf{+2.2} &\bf{48.4}\gbf{+1.6} &\bf{30.3}\gbf{+2.7} &\bf{26.5}\gbf{+1.8} &\bf{45.3}\gbf{+1.7} &\bf{27.3}\gbf{+2.0} &27.9\rbf{-0.5} &46.9\rbf{-1.4} &29.3\rbf{-0.2} &26.0\rbf{-0.4} &44.2\rbf{-1.0} &\bf{26.9}\gbf{+1.2} \\ 
% DetCo+AA &\bf{29.8}\gbf{+2.7} &\bf{49.1}\gbf{+2.3} &\bf{31.4}\gbf{+3.8} &\bf{26.9}\gbf{+2.2} &\bf{46.0}\gbf{+2.4} &\bf{27.9}\gbf{+2.6} &\bf{29.6}\gbf{+1.2} &\bf{49.4}\gbf{+1.1} &\bf{31.0}\gbf{+1.5} &\bf{27.6}\gbf{+1.2} &\bf{46.6}\gbf{+1.4} &\bf{28.7}\gbf{+3.0} \\
DetCo &\bf{29.8}\gbf{+2.7} &\bf{49.1}\gbf{+2.3} &\bf{31.4}\gbf{+3.8} &\bf{26.9}\gbf{+2.2} &\bf{46.0}\gbf{+2.4} &\bf{27.9}\gbf{+2.6} &\bf{29.6}\gbf{+1.2} &\bf{49.4}\gbf{+1.1} &\bf{31.0}\gbf{+1.5} &\bf{27.6}\gbf{+1.2} &\bf{46.6}\gbf{+1.4} &\bf{28.7}\gbf{+3.0} \\

\end{tabular}}
\caption{\small{
\textbf{Object detection and instance segmentation fine-tuned on COCO}. All methods are pretrained 200 epochs on ImageNet. \textbf{\green{Green}} means increase and \textbf{\gray{gray}} means decrease. DetCo outperforms all supervised and unsupervised counterparts.  
% ``AA'' means we use Auto Augmentation in pre-training.
}
}

\label{tab:coco_12k_c4fpn}
% \vspace{-3mm}
\end{table*}

==> LaTeX/tables/table_c4_fpn_180k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|l l l |l l l |l l l}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-C4 COCO 180k} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 180k} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &35.6           &54.6           &38.2           &31.4           &51.5           &33.5           &36.7           &56.7           &40.0           &33.7           &53.8           &35.9 \\
Supervised   &40.0           &59.9           &43.1           &34.7           &56.5           &36.9           &40.6           &61.3           &44.4           &36.8           &58.1           &39.5 \\ \hline
MoCo\cite{moco}      &40.7\gbf{+0.7} &60.5\gbf{+0.6} &44.1\gbf{+1.0} &35.4\gbf{+0.7} &57.3\gbf{+0.8} &37.6\gbf{+0.7} &40.8\gbf{+0.2} &61.6\gbf{+0.3} &44.7\gbf{+0.3} &36.9\gbf{+0.1} &58.4\gbf{+0.3} &39.7\gbf{+0.2} \\ 
MoCov2\cite{mocov2}      &41.0\gbf{+1.0} &60.6\gbf{+0.7} &44.5\gbf{+1.4} &35.6\gbf{+0.9} &57.2\gbf{+0.7} &38.0\gbf{+1.1} &40.9\gbf{+0.3} &61.5\gbf{+0.2} &44.7\gbf{+0.3} &37.0\gbf{+0.2} &58.7\gbf{+0.6} &39.8\gbf{+0.3} \\ \hline
% DetCo        &\bf{41.4}\gbf{+1.4} &\bf{61.2}\gbf{+1.3} &\bf{44.7}\gbf{+1.6} &\bf{35.8}\gbf{+1.1} &\bf{57.8}\gbf{+1.3} &\bf{38.3}\gbf{+1.4} &\bf{41.5}\gbf{+0.9} &\bf{62.1}\gbf{+0.8} &\bf{45.6}\gbf{+1.2} &\bf{37.6}\gbf{+0.8} &\bf{59.2}\gbf{+1.1} &\bf{40.5}\gbf{+1.0} \\ 
% DetCo+AA     &\bf{41.3}\gbf{+1.3} &\bf{61.2}\gbf{+1.3} &\bf{45.0}\gbf{+1.9} &\bf{35.8}\gbf{+1.1} &\bf{57.9}\gbf{+1.4} &\bf{38.2}\gbf{+1.3} &\bf{41.5}\gbf{+0.9} &\bf{62.5}\gbf{+1.2} &\bf{45.6}\gbf{+1.2} &\bf{37.7}\gbf{+0.9} &\bf{59.5}\gbf{+1.4} &\bf{40.5}\gbf{+1.0} \\ 
DetCo    &\bf{41.3}\gbf{+1.3} &\bf{61.2}\gbf{+1.3} &\bf{45.0}\gbf{+1.9} &\bf{35.8}\gbf{+1.1} &\bf{57.9}\gbf{+1.4} &\bf{38.2}\gbf{+1.3} &\bf{41.5}\gbf{+0.9} &\bf{62.5}\gbf{+1.2} &\bf{45.6}\gbf{+1.2} &\bf{37.7}\gbf{+0.9} &\bf{59.5}\gbf{+1.4} &\bf{40.5}\gbf{+1.0} \\ 

\end{tabular}}
\caption{\textbf{Object detection and instance segmentation fine-tuned on COCO}. 
All methods are pretrained 200 epochs on ImageNet.
DetCo outperforms all supervised and unsupervised counterparts. 
}
\label{tab:coco_180k_c4fpn}
\end{table*}

==> LaTeX/tables/table_c4_fpn_90k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|l l l |l l l |l l l |l l l}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-C4 COCO 90k} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 90k} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &26.4 &44.0 &27.8 &29.3 &46.9 &30.8 &31.0 &49.5 &33.2 &28.5 &46.8 &30.4 \\
Supervised  &38.2 &58.2 &41.2 &33.3 &54.7 &35.2 &38.9 &59.6 &42.7 &35.4 &56.5 &38.1  \\ \hline
InsDis\cite{wu2018unsupervised}      & 37.7\rbf{-0.5} & 57.0\rbf{-1.2} & 40.9\rbf{-0.3} & 33.0\rbf{-0.3} & 54.1\rbf{-0.6} & 35.2\rbf{0.0} & 37.4\rbf{-1.5} & 57.6\rbf{-2.0}  & 40.6\rbf{-2.1} &34.1\rbf{-1.3} & 54.6\rbf{-1.9} & 36.4\rbf{-1.7} \\
PIRL\cite{pirl}        & 37.4\rbf{-0.8} & 56.5\rbf{-1.7} & 40.2\rbf{-1.0} & 32.7\rbf{-0.6} & 53.4\rbf{-1.3} & 34.7\rbf{-0.5} & 37.5\rbf{-1.4} & 57.6\rbf{-2.0} & 41.0\rbf{-1.7} &34.0\rbf{-1.4} & 54.6\rbf{-1.9} & 36.2\rbf{-1.9} \\ 
SwAV\cite{swav}        & 32.9\rbf{-5.3} & 54.3\rbf{-3.9} & 34.5\rbf{-6.7} & 29.5\rbf{-3.8} & 50.4\rbf{-4.3} & 30.4\rbf{-4.8} & 38.5\rbf{-0.4} & 60.4\gbf{+0.8} & 41.4\rbf{-1.3} &35.4\rbf{0.0}  & 57.0\gbf{+0.5} & 37.7\rbf{-0.4} \\ 
MoCo\cite{moco}     &38.5\gbf{+0.3} &58.3\gbf{+0.1} &41.6\gbf{+0.4} &33.6\gbf{+0.3} &54.8\gbf{+0.1} &35.6\gbf{+0.4} &38.5\rbf{-0.4} &58.9\rbf{-0.7}         & 42.0\rbf{-0.7} &35.1\rbf{-0.3} & 55.9\rbf{-0.6} &37.7\rbf{-0.4} \\ 
MoCov2\cite{mocov2}     &38.9\gbf{+0.7} &58.4\gbf{+0.2} &42.0\gbf{+0.8} &34.2\gbf{+0.9} &55.2\gbf{+0.5} &36.5\gbf{+1.3} &38.9\rbf{0.0}  &59.4\rbf{-0.2}         &42.4\rbf{-0.3}  &35.5\gbf{+0.1} & 56.5\rbf{0.0} &38.1\rbf{0.0} \\ \hline
% DetCo      &\bf{39.4}\gbf{+1.2} &\bf{59.2}\gbf{+1.0} &\bf{42.3}\gbf{+1.1} &\bf{34.4}\gbf{+1.1} &\bf{55.7}\gbf{+1.0} &\bf{36.6}\gbf{+1.4} &\bf{39.5}\gbf{+0.6} &60.3\gbf{+0.7}         &\bf{43.1}\gbf{+0.4}  &\bf{35.9}\gbf{+0.5} & 56.9\gbf{+0.4} &\bf{38.6}\gbf{+0.5} \\ 
% DetCo+AA      &\bf{39.8}\gbf{+1.6} &\bf{59.7}\gbf{+1.5} &\bf{43.0}\gbf{+1.8} &\bf{34.7}\gbf{+1.4} &\bf{56.3}\gbf{+1.6} &\bf{36.7}\gbf{+1.5} &\bf{40.1}\gbf{+1.2} &\bf{61.0}\gbf{+1.4}         &\bf{43.9}\gbf{+1.2}  &\bf{36.4}\gbf{+1.0} & \bf{58.0}\gbf{+1.5} &\bf{38.9}\gbf{+0.8} \\ 
DetCo      &\bf{39.8}\gbf{+1.6} &\bf{59.7}\gbf{+1.5} &\bf{43.0}\gbf{+1.8} &\bf{34.7}\gbf{+1.4} &\bf{56.3}\gbf{+1.6} &\bf{36.7}\gbf{+1.5} &\bf{40.1}\gbf{+1.2} &\bf{61.0}\gbf{+1.4}         &\bf{43.9}\gbf{+1.2}  &\bf{36.4}\gbf{+1.0} & \bf{58.0}\gbf{+1.5} &\bf{38.9}\gbf{+0.8} \\ 
\end{tabular}}
\caption{\small{
\textbf{Object detection and instance segmentation fine-tuned on COCO}. 
All methods are pretrained 200 epochs on ImageNet.
DetCo outperforms all supervised and unsupervised counterparts. 
% ``AA'' means we use Auto Augmentation in pre-training.
}
}
\label{tab:coco_90k_c4fpn}
\vspace{-3mm}
\end{table*}

==> LaTeX/tables/table_c4_fpn_percent1_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|lll|lll|lll}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-FPN COCO 1\% Data} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 2\% Data} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &2.5 &5.8 &1.7 &2.3 &4.9 &1.8 &4.5 &10.3 &3.2 &4.3 &9.3 &3.5 \\
Supervised       &10.0 &19.9 &9.2 &9.7 &18.3 &9.2 &13.7 &26.6 &12.8 &13.0 &24.2 &12.6 \\ \hline
MoCo\cite{moco}             &9.1\rbf{-0.9} &17.3\rbf{-2.6} &8.6\rbf{-0.6} &8.6\rbf{-1.1} &16.1\rbf{-2.2} &8.3\rbf{-0.9} &13.0\rbf{-0.7} &24.1\rbf{-2.5} &12.6\rbf{-0.2} &12.3\rbf{-0.7} &22.4\rbf{-1.8} &12.2\rbf{-0.4} \\
MoCo v2\cite{mocov2}          &9.9\rbf{-0.1}& 18.7\rbf{-1.2} &9.5\gbf{+0.3} &9.5\rbf{-0.2} &17.2\rbf{-1.1} &9.2\rbf{0.0} &13.8\gbf{+0.1} &25.3\rbf{-1.3} &13.4\gbf{+0.6} &12.9\rbf{-0.1} &23.3\rbf{-0.9} &12.7\gbf{+0.1} \\ \hline
% DetCo            &\textbf{10.7}\gbf{+0.7} &\textbf{20.2}\gbf{+0.3} &\textbf{10.4}\gbf{+1.2} &\textbf{10.2}\gbf{+0.5} & \textbf{19.0}\gbf{+0.7} &\textbf{9.9}\gbf{+0.7} &\textbf{14.3}\gbf{+0.6} &\textbf{26.3}\rbf{-0.3} &\textbf{13.9}\gbf{+1.1} &\textbf{13.5}\gbf{+0.5} &\textbf{24.6}\gbf{+0.4} &\textbf{13.1}\gbf{+0.5}\\
% DetCo+AA         &\textbf{12.4}\gbf{+2.4} &\textbf{23.5}\gbf{+3.6} &\textbf{11.8}\gbf{+2.6} &\textbf{12.1}\gbf{+2.4} & \textbf{21.9}\gbf{+3.6} &\textbf{12.0}\gbf{+2.8} &\textbf{16.0}\gbf{+2.3} &\textbf{29.6}\gbf{+3.0} &\textbf{15.6}\gbf{+2.8} &\textbf{15.3}\gbf{+2.3} &\textbf{27.4}\gbf{+2.2} &\textbf{15.1}\gbf{+2.5}\\
DetCo         &\textbf{12.4}\gbf{+2.4} &\textbf{23.5}\gbf{+3.6} &\textbf{11.8}\gbf{+2.6} &\textbf{12.1}\gbf{+2.4} & \textbf{21.9}\gbf{+3.6} &\textbf{12.0}\gbf{+2.8} &\textbf{16.0}\gbf{+2.3} &\textbf{29.6}\gbf{+3.0} &\textbf{15.6}\gbf{+2.8} &\textbf{15.3}\gbf{+2.3} &\textbf{27.4}\gbf{+2.2} &\textbf{15.1}\gbf{+2.5}\\

 

\end{tabular}}
\caption{\small{
\textbf{Semi-Supervised two-stage Detection fine-tuned on COCO 1\% and 2\% data}. All methods are pretrained 200 epochs on ImageNet. \textbf{\green{Green}} means increase and \textbf{\gray{gray}} means decrease. DetCo is better than supervised~/~unsupervised counterparts in all metrics.
}
}

\label{tab:coco_1_2_c4fpn}
\end{table*}

==> LaTeX/tables/table_c4_fpn_percent5_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|lll|lll|lll}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-FPN COCO 5\% Data} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 10\% Data} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &9.2& 18.6& 7.9& 8.8& 16.9& 8.1 &10.1& 20.2& 9.1& 9.8& 18.6& 9.2 \\
Supervised       &19.9& 37.0& 19.3& 18.6& 33.7& 18.4 &23.8& 42.8& 23.9& 22.2& 39.6& 22.3 \\ \hline
MoCo\cite{moco}             &19.6\rbf{-0.3} &35.1\rbf{-1.9} &20.0\gbf{+0.7} &18.3\rbf{-0.3} &32.3\rbf{-1.4} &18.6\gbf{+0.2} &23.3\rbf{-0.5} &40.7\rbf{-2.1} &23.9\rbf{0.0} &21.9\rbf{-0.3} &38.0\rbf{-1.6} &22.4\gbf{+0.1} \\
MoCo v2\cite{mocov2}          &20.6\gbf{+0.7} &36.6\rbf{-0.4} &21.0\gbf{+1.7} &19.1\gbf{+0.5} &33.7\rbf{0.0} &19.2\gbf{+0.8} &24.1\gbf{+0.3} &42.0\rbf{-0.8} &24.8\gbf{+0.9} &22.5\gbf{+0.3} &39.1\rbf{-0.5} &23.3\gbf{+1.0} \\ \hline
% DetCo            &\textbf{21.4}\gbf{+1.5} &\textbf{38.1}\gbf{+1.1} &\textbf{21.6}\gbf{+2.3} &\textbf{19.9}\gbf{+1.3} &\textbf{35.1}\gbf{+1.4} &\textbf{19.8}\gbf{+1.4} &\textbf{25.3}\gbf{+1.5} &\textbf{43.9}\gbf{+1.1} &\textbf{26.0}\gbf{+2.1} &\textbf{23.6}\gbf{+1.4} &\textbf{40.8}\gbf{+1.2} &\textbf{24.0}\gbf{+1.7} \\
% DetCo+AA        &\textbf{21.9}\gbf{+2.0} &\textbf{39.1}\gbf{+2.1} &\textbf{22.2}\gbf{+2.9} &\textbf{20.4}\gbf{+1.8} &\textbf{36.1}\gbf{+2.4} &\textbf{20.6}\gbf{+2.2} &\textbf{26.0}\gbf{+2.2} &\textbf{45.2}\gbf{+2.4} &\textbf{27.0}\gbf{+3.1} &\textbf{24.3}\gbf{+2.1} &\textbf{42.0}\gbf{+2.4} &\textbf{25.0}\gbf{+2.7} \\
DetCo        &\textbf{21.9}\gbf{+2.0} &\textbf{39.1}\gbf{+2.1} &\textbf{22.2}\gbf{+2.9} &\textbf{20.4}\gbf{+1.8} &\textbf{36.1}\gbf{+2.4} &\textbf{20.6}\gbf{+2.2} &\textbf{26.0}\gbf{+2.2} &\textbf{45.2}\gbf{+2.4} &\textbf{27.0}\gbf{+3.1} &\textbf{24.3}\gbf{+2.1} &\textbf{42.0}\gbf{+2.4} &\textbf{25.0}\gbf{+2.7} \\

\end{tabular}}
\caption{\small{
\textbf{Semi-Supervised two-stage Detection fine-tuned on COCO 5\% and 10\% data}. All methods are pretrained 200 epochs on ImageNet. DetCo is better than supervised~/~unsupervised counterparts in all metrics.
}
}

\label{tab:coco_5_10_c4fpn}
\end{table*}

==> LaTeX/tables/table_city.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\scalebox{0.93}{
\begin{tabular}{l|l l|l}
% \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{Instance Seg.} & \multicolumn{1}{c}{Semantic Seg.} \\ \cline{2-4} 
 & \multicolumn{1}{l}{AP$^{mk}$} & \multicolumn{1}{l|}{AP$_{50}^{mk}$} & \multicolumn{1}{l}{mIOU} \\ \shline
\gray{Rand Init} & 25.4 & 51.1 & 65.3 \\ 
supervised   & 32.9                & 59.6                 & 74.6 \\ \hline
InsDis~\cite{wu2018unsupervised}     & 33.0~\gbf{+0.1} & 60.1~\gbf{+0.5}  & 73.3~\rbf{-1.3} \\ 
PIRL~\cite{pirl}         & 33.9~\gbf{+1.0} & 61.7~\gbf{+2.1}   & 74.6~\rbf{0.0} \\ 
SwAV~\cite{swav}         & 33.9~\gbf{+1.0} & 62.4~\gbf{+2.8}  & 73.0~\rbf{-1.6} \\ 
MoCo~\cite{moco}      & 32.3~\rbf{-0.6}   & 59.3~\rbf{-0.3}    & 75.3~\gbf{+0.7} \\ 
MoCov2~\cite{mocov2}      & 33.9~\gbf{+1.0} & 60.8~\gbf{+1.2}  & 75.7~\gbf{+1.1} \\ \hline
DetCo        & \bf{34.7}~\gbf{+1.8} & \bf{63.2}~\gbf{+3.6}  & \bf{76.5}~\gbf{+1.9} \\ 
% \hline
\end{tabular}}
\caption{\textbf{DetCo \textit{vs.} supervised and other unsupervised methods on Cityscapes dataset.} 
All methods are pretrained 200 epochs on ImageNet.
We evaluate instance segmentation and semantic segmentation tasks.}\label{tab:city}
\vspace{-3mm}
\end{table}

==> LaTeX/tables/table_imagenet.tex <==
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{l|c|cc|c}
% Method & Epoch & Top1 & Top5 & VOC Cls. \\ \cline{1-5}
\multirow{2}{*}{Method} & \multirow{2}{*}{Epoch} & \multicolumn{2}{c|}{ImageNet} & VOC07 \\ \cline{3-5} 
 & & \multicolumn{1}{c}{Top1} & Top5 & \multicolumn{1}{c}{Acc} \\ \shline
% Exemplar & - & 46.0 & - &- \\
% Rel-Loc & - & 51.4 & - &- \\
Jigsaw~\cite{noroozi2016unsupervised} & - & 44.6 & - &64.5 \\
Rotation~\cite{gidaris2018unsupervised} & - & 55.4 &- & 63.9 \\
% DeepCluster & - & 48.4 & - & \\
% BigBiGAN & - & 56.6 & - &- \\
InsDis~\cite{wu2018unsupervised} & 200 & 56.5 & - &76.6 \\
LocalAgg~\cite{localagg} & 200 & 58.8 & - &- \\
% CPC v2 & - & 63.8 & 85.3 &- \\
PIRL~\cite{pirl} & 800 & 63.6 &- &81.1 \\
SimCLR~\cite{simclr} & 1000 & 69.3 & 89.0 &- \\
BYOL~\cite{byol} & 1000 & 74.3 & 91.6 & -\\
SwAV~\cite{swav} & 200 & 72.7 & - & 87.6\\
MoCo~\cite{moco} & 200 & 60.6 & - &79.2 \\ 
MoCov2~\cite{mocov2} & 200 & 67.5 & -  & 84.1\\ \hline
%  & 800 & 71.1 & - &87.1 \\ \cline{1-5}
DetCo & 200 & 68.6 & 88.5 &85.1 \\
%  & 800 & ? & ? &87.1 \\ 
\end{tabular}}
\caption{\textbf{Comparison  of ImageNet Linear Classification and VOC SVM Classification.} Although DetCo is designed for detection, it is also robust and competitive on classification task, and it substantially exceeds MoCov2 baseline by 1.1\%.
} % end caption
\label{tab:results_imgnet}
% \vspace{-3mm}
\end{table}

==> LaTeX/tables/table_lvis.tex <==
\begin{table}[]
\centering
\scalebox{0.90}{
\begin{tabular}{l|ccc|ccc}
Method     & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \hline
\gray{Rand Init}  & 19.6 & 31.8   & 20.9   & 19.0 & 29.8   & 20.1   \\ 
Supervised & 22.7 & 36.8   & 24.1   & 22.2 & 34.6   & 23.5   \\ \hline
MoCo\cite{moco}   & 23.1 & 37.4   & 24.5   & 22.5 & 35.1   & 23.8   \\ 
MoCo v2\cite{mocov2}    & 23.2 & 37.4   & 24.7   & 22.8 & 35.1   & 24.4   \\ \hline
DetCo      & \bf{23.5} & \bf{37.7}   & \bf{24.8}   & \bf{23.0} & \bf{35.5}   & \bf{24.5}   \\ 
\end{tabular}}
\caption{\textbf{DetCo \textit{vs.} supervised and other unsupervised methods on LVIS v1.0 dataset.} 
All methods are pretrained 200 epochs on ImageNet.
We evaluate object detection and instance segmentation tasks.}
\label{tab:lvis}
\vspace{-5mm}
\end{table}

==> LaTeX/tables/table_mesh.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|c|l|l|l}
Method       & Epoch & AP$^{dp}$ & AP$^{dp}_{50}$ & AP$^{dp}_{75}$ \\ \shline
\gray{Rand Init} & -          &40.8             &78.6            &37.3       \\ 
Supervised   & 90             &50.8             &86.3            &52.6 \\ \hline
MoCo~\cite{moco}      & 200   &49.6\rbf{-1.2}  &85.9\rbf{-0.4} &50.5\rbf{-2.1}       \\ 
MoCo v2~\cite{mocov2} & 200   &50.9\gbf{+0.1}  &87.2\gbf{+0.9} &52.9\gbf{+0.3}       \\  \hline
DetCo        & 200   &\bf{51.3}\gbf{+0.5}           &\bf{87.7}\gbf{+1.4} &\bf{53.3}\gbf{+0.7} \\ 
\end{tabular}}
\caption{\textbf{DetCo \textit{vs.} other methods on Dense Pose task.} It also performs best on monocular 3D human shape prediction.}
% \vspace{-3mm}
\label{tab:dprcnn}
\end{table}

==> LaTeX/tables/table_retina_percent_1_2_5_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|lll|lll|lll}
\multirow{2}{*}{Method} &\multicolumn{3}{c|}{RetinaNet R50 COCO 1\% Data} &\multicolumn{3}{c|}{RetinaNet R50 COCO 2\% Data} &\multicolumn{3}{c|}{RetinaNet R50 COCO 5\% Data} &\multicolumn{3}{c}{RetinaNet R50 COCO 10\% Data} \\ \cline{2-13} 
 &AP &AP$_{50}$ &AP$_{75}$ &AP &AP$_{50}$ &AP$_{75}$  &AP &AP$_{50}$ &AP$_{75}$ &AP &AP${50}$ &AP${75}$ \\ \shline
\gray{Rand Init}     &1.4  &3.5  &1.0 &2.5  &5.6  &2.0  &3.6  &7.4   &3.0   &3.7  &7.5  &3.2 \\ 
Supervised           &8.2  &16.2 &7.2 &11.2 &21.7 &10.3 &16.5 &30.3  &15.9  &19.6 &34.5 &19.7 \\ \hline
MoCo\cite{moco}                 &7.0\rbf{-1.2} &13.5\rbf{-2.7} &6.5\rbf{-0.7} &10.3\rbf{-0.9} &19.2\rbf{-2.5} &9.7\rbf{-0.6} &15.0\rbf{-1.5} &27.0\rbf{-3.3} &14.9\rbf{-1.0} &18.2\rbf{-1.4} &31.6\rbf{-2.9} &18.4\rbf{-1.3} \\
MoCo v2\cite{mocov2}              &8.4\gbf{+0.2} &15.8\rbf{-0.4} &8.0\gbf{+0.8} &12.0\gbf{+0.8} &21.8\gbf{+0.1} &11.5\gbf{+1.2} &16.8\gbf{+0.3} &29.6\rbf{-0.7} &16.8\gbf{+0.9} &20.0\gbf{+0.4} &34.3\rbf{-0.2} &20.2\gbf{+0.5} \\ \hline
% DetCo                &\textbf{8.8}\gbf{+0.6} &\textbf{16.7}\gbf{+0.5} &\textbf{8.2}\gbf{+1.0} &\textbf{13.0}\gbf{+1.8} &\textbf{24.0}\gbf{+2.3} &\textbf{12.5}\gbf{+2.2} &\textbf{17.9}\gbf{+1.4} &\textbf{31.7}\gbf{+1.4} &\textbf{17.7}\gbf{+1.8} &\textbf{20.8}\gbf{+1.2} &\textbf{35.6}\gbf{+1.1} &\textbf{21.3}\gbf{+1.6} \\
DetCo            &\textbf{9.9}\gbf{+1.7} &\textbf{19.3}\gbf{+3.1} &\textbf{9.1}\gbf{+1.9} &\textbf{13.5}\gbf{+2.3} &\textbf{25.1}\gbf{+3.4} &\textbf{12.7}\gbf{+2.4} &\textbf{18.7}\gbf{+2.2} &\textbf{32.9}\gbf{+2.6} &\textbf{18.7}\gbf{+2.8} &\textbf{21.9}\gbf{+2.3} &\textbf{37.6}\gbf{+3.1} &\textbf{22.3}\gbf{+2.6} 


\end{tabular}}
\caption{\small{
\textbf{Semi-Supervised one-stage detection fine-tuned on COCO 1\%, 2\%, 5\% and 10\%  data}. All methods are pretrained 200 epochs on ImageNet. 
DetCo is significant better than supervised~/~unsupervised counterparts in all metrics.
}
}
\label{tab:retina_1_2_5_10}
\end{table*}

==> LaTeX/tables/table_retina_pose.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|l l l |l l l |l l l |l l l}
% \hline
\multirow{2}{*}{Method} &\multicolumn{3}{c|}{RetinaNet R50 12k} &\multicolumn{3}{c|}{RetinaNet R50 90k} &\multicolumn{3}{c|}{RetinaNet R50 180k} &\multicolumn{3}{c}{Keypoint RCNN R50 180k} \\ \cline{2-13} 
 &AP &AP$_{50}$ &AP$_{75}$ &AP &AP$_{50}$ &AP$_{75}$  &AP &AP$_{50}$ &AP$_{75}$ &AP$^{kp}$ &AP$^{kp}_{50}$ &AP$^{kp}_{75}$ \\ \shline
\gray{Rand Init} &4.0            &7.9            &3.5            &24.5           &39.0           &25.7           &32.2            &49.4            &34.2            &65.9           &86.5           &71.7 \\ 
Supervised  &24.3           &40.7           &25.1           &37.4           &56.5           &39.7           &38.9            &58.5            &41.5            &65.8           &86.9           &71.9 \\ \hline
InsDis\cite{wu2018unsupervised} &19.0\rbf{-5.3} &32.0\rbf{-8.7} &19.6\rbf{-5.5} &35.5\rbf{-1.9} &54.1\rbf{-2.4} &38.2\rbf{-1.5} &38.0\rbf{-0.9}  &57.4\rbf{-1.1}  &40.5\rbf{-1.0}  &66.5\gbf{+0.7} &87.1\gbf{+0.2} &72.6\gbf{+0.7} \\ 
PIRL\cite{pirl}        &19.0\rbf{-5.3} &31.7\rbf{-9.0} &19.8\rbf{-5.3} &35.7\rbf{-1.7} &54.2\rbf{-2.3} &38.4\rbf{-1.3} &38.5\rbf{-0.4}  &57.6\rbf{-0.9}  &41.2\rbf{-0.3}  &66.5\gbf{+0.7} &87.5\gbf{+0.6} &72.1\gbf{+0.2} \\ 
SwAV\cite{swav}        &19.7\rbf{-4.6} &34.7\rbf{-6.0} &19.5\rbf{-5.6} &35.2\rbf{-2.2} &54.9\rbf{-1.6} &37.5\rbf{-2.2} &38.6\rbf{-0.3}  &58.8\gbf{+0.3}  &41.1\rbf{-0.4}  &66.0\gbf{+0.2} &86.9\rbf{0.0}  &71.5\rbf{-0.4} \\ 
MoCo\cite{moco}     &20.2\rbf{-4.1} &33.9\rbf{-6.8} &20.8\rbf{-4.3} &36.3\rbf{-1.1} &55.0\rbf{-1.5} &39.0\rbf{-0.7} &38.7\rbf{-0.2}  &57.9\rbf{-0.6}  &41.5\rbf{0.0}   &66.8\gbf{+1.0} &87.4\gbf{+0.5} &72.5\gbf{+0.6} \\ 
MoCov2\cite{mocov2}     &22.2\rbf{-2.1} &36.9\rbf{-3.8} &23.0\rbf{-2.1} &37.2\rbf{-0.2} &56.2\rbf{-0.3} &39.6\rbf{-0.1} &39.3\gbf{+0.4}  &58.9\gbf{+0.4}  &42.1\gbf{+0.6}  &66.8\gbf{+1.0} &87.3\gbf{+0.4} &73.1\gbf{+1.2} \\ \hline
% DetCo      &23.6\rbf{-0.7} &38.7\rbf{-2.0} &24.6\rbf{-0.5} &\bf{38.0}\gbf{+0.6} &\bf{57.4}\gbf{+0.9} &\bf{40.7}\gbf{+1.0} &\bf{39.8}\gbf{+0.9}  &\bf{59.5}\gbf{+1.0}  &\bf{42.4}\gbf{+0.9}  &\bf{67.2}\gbf{+1.4} &\bf{87.5}\gbf{+0.6} &\bf{73.4}\gbf{+1.5} \\ 
% DetCo+AA          &\bf{25.3}\gbf{+1.0} &\bf{41.6}\gbf{+0.9} &\bf{26.5}\gbf{+1.4} &\bf{38.4}\gbf{+1.0} &\bf{57.8}\gbf{+1.3} &\bf{41.2}\gbf{+1.5} &\bf{39.7}\gbf{+0.8}  &\bf{59.3}\gbf{+0.8}  &\bf{42.6}\gbf{+1.1}  &- &- &- \\ 
DetCo          &\bf{25.3}\gbf{+1.0} &\bf{41.6}\gbf{+0.9} &\bf{26.5}\gbf{+1.4} &\bf{38.4}\gbf{+1.0} &\bf{57.8}\gbf{+1.3} &\bf{41.2}\gbf{+1.5} &\bf{39.7}\gbf{+0.8}  &\bf{59.3}\gbf{+0.8}  &\bf{42.6}\gbf{+1.1}  &\bf{67.2}\gbf{+1.4} &\bf{87.5}\gbf{+0.6} &\bf{73.4}\gbf{+1.5} \\ 

\end{tabular}}
\caption{\small{
\textbf{One-stage object detection and keypoint detection fine-tuned on COCO}. 
All methods are pretrained 200 epochs on ImageNet.
DetCo outperforms all supervised and unsupervised counterparts. 
% ``AA'' means we use Auto Augmentation in pre-training.
}
}
\label{tab:retina_pose}
% \vspace{-5mm}
\end{table*}

==> LaTeX/tables/table_vocdet.tex <==
\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|c|l l l}
Method & Epoch & AP & AP$_{50}$ & AP$_{75}$ \\ \shline
\gray{Rand Init} & - &33.8 &60.2 &33.1 \\ 
Supervised                       & 90  &53.5           &81.3           &58.8 \\ \hline
InsDis~\cite{wu2018unsupervised} & 200 &55.2\gbf{+1.7} &80.9\rbf{-0.4} &61.2\gbf{+2.4} \\ 
PIRL~\cite{pirl}                 & 200 &55.5\gbf{+2.0} &81.0\rbf{-0.3} &61.3\gbf{+2.5} \\ 
SwAV~\cite{swav}                 & 800 &56.1\gbf{+2.6} &82.6\gbf{+1.3} &62.7\gbf{+3.9} \\ 
MoCo~\cite{moco}                 & 200 &55.9\gbf{+2.4} &81.5\gbf{+0.2} &62.6\gbf{+3.8} \\ 
MoCov2~\cite{mocov2}             & 200 &57.0\gbf{+3.5} &82.4\gbf{+1.1} &63.6\gbf{+4.8} \\ 
MoCov2~\cite{mocov2}             & 800 &57.4\gbf{+3.9} &82.5\gbf{+1.2} &64.0\gbf{+5.2} \\ \hline
DetCo                            & 100 &57.4\gbf{+3.9} &82.5\gbf{+1.2} &63.9\gbf{+5.1} \\ 
                            & 200 &57.8\gbf{+4.3} &82.6\gbf{+1.3} &64.2\gbf{+5.4} \\ 
                            & 800 &\bf{58.2}\gbf{+4.7} &\bf{82.7}\gbf{+1.4} &\bf{65.0}\gbf{+6.2} \\ 
\end{tabular}}
\caption{\textbf{Object Detection finetuned on PASCAL VOC07+12 using Faster RCNN-C4.} DetCo-100ep is on par with previous state-of-the-art, and DetCo-800ep achieves the best performance.
}
\label{tab:voc}
% \vspace{-3mm}
\end{table}

==> tables/ablation_1_new.tex <==
% \begin{table}[h]
% \centering
% \scalebox{0.7}{
\begin{tabular}{c|c|c|l l|l}
% \hline
 & +HIC & +CGLC & Top1 & Top5 & mAP \\ \shline
(a) & $\times$ & $\times$ & 64.3 & 85.6 & 56.3 \\ \shline
(b) & \checkmark & $\times$ & 63.2~$\red{\pmb{\downarrow}}$ & 84.9~$\red{\pmb{\downarrow}}$ & 57.0~$\green{\pmb{\uparrow}}$ \\ \hline
(c) & $\times$ &  \checkmark & 67.1~$\green{\pmb{\uparrow}}$ & 87.5~$\green{\pmb{\uparrow}}$ & 56.8~$\green{\pmb{\uparrow}}$ \\ \hline
(d) & \checkmark & \checkmark & 66.6~$\green{\pmb{\uparrow}}$ & 87.2~$\green{\pmb{\uparrow}}$ & 57.4~$\green{\pmb{\uparrow}}$ \\ 
\end{tabular}
% \caption{
% }
% \label{tab:ab1_new}
% \vspace{-3mm}
% \end{table}

==> tables/ablation_2_new.tex <==
% \begin{table}[h]
% \centering
% \scalebox{0.65}{
\begin{tabular}{c|c|c|l l l l}

    & +HIC & +CGLC & Res2 & Res3 & Res4 & Res5 \\ \shline
(a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1 \\ \shline
(b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$ \\ \hline
(c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \hline
(d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$ \\ 
\end{tabular}
% }
% \caption{}
% \label{tab:ab2_new}
% \vspace{-5mm}
% \end{table}

==> tables/ablation_3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\scalebox{0.85}{
\begin{tabular}{l|l|ccc}
    & weight                          & AP   & AP$_{50}$ & AP$_{75}$ \\ \shline
(a) & (0,0,0,1) & 56.3 & 81.8 & 62.1 \\
(b) & (1,1,1,1)+Norm                  & 55.1 & 80.4 & 60.4 \\
(c) & (1,1,1,1)                       & 55.8 & 81.6 & 62.2 \\
(d) & (0.1,0.4,0.7,1)+Norm            & 56.5 & 82.2 & 62.7 \\
(e) & (0.1,0.4,0.7,1)                 & 57.0 & 82.2 & 63.1
\end{tabular}}
\caption{Ablation study of intermediate loss weight, under 100 epoch pre-training. ``Norm'' means normalized the loss weights, making the sum of weights equals 1.0.}
\label{tab:ab3}
\end{table}

==> tables/ablation_4.tex <==
\begin{table}[]
\centering
\scalebox{1.0}{
\begin{tabular}{l|c|ccc}
    & share queue & AP   & AP$_{50}$ & AP$_{75}$ \\ \shline
(a) & \checkmark           & 56.2 & 81.8 & 62.3 \\
(b) & $\times$           & 57.0 & 82.2 & 63.1
\end{tabular}}
\caption{Ablation study of share or not share queue, under 100 epoch pre-training.}
\label{tab:ab4}
\end{table}

==> tables/ablation_5.tex <==
\begin{table}[]
\centering
\scalebox{1.0}{
\begin{tabular}{l|c|c|c|c}
    & $+\mathcal{L}_{g \leftrightarrow g}$ & $+\mathcal{L}_{g \leftrightarrow l}$ & $+\mathcal{L}_{l \leftrightarrow l}$ & AP   \\ \shline
(a) & \checkmark    & $\times$    & $\times$    & 56.0 \\
(b) & \checkmark    & \checkmark    & $\times$    & 56.2 \\
(c) & \checkmark    & \checkmark    & \checkmark    & 56.5
\end{tabular}}
\caption{Ablation study of cross contrastive loss, under 50 epoch pre-training.}
\label{tab:ab5}
\end{table}

==> tables/ablation_both_new.tex <==

\begin{tabular}{p{12pt}<{\centering}|p{20pt}<{\centering}|p{27pt}<{\centering}|p{20pt}<{\centering} p{20pt}<{\centering}|p{20pt}<{\centering} p{5pt}<{\centering} p{12pt}<{\centering}|p{20pt}<{\centering}|p{27pt}<{\centering}|p{20pt}<{\raggedright}p{20pt}<{\raggedright}p{20pt}<{\raggedright}p{20pt}<{\raggedright}}
% \hline
 & +HIC & +CGLC & Top1 & Top5 & mAP & & & +HIC & +CGLC & Res2 & Res3 & Res4 & Res5 \\ \cline{1-6}\cline{8-14}
 
\rule{0pt}{10pt}(a) & $\times$ & $\times$ & 64.3 & 85.6 & 56.3 & & (a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1\\ \cline{1-6}\cline{8-14}

\rule{0pt}{10pt}(b) & \checkmark & $\times$ & 63.2~$\red{\pmb{\downarrow}}$ & 84.9~$\red{\pmb{\downarrow}}$ & 57.0~$\green{\pmb{\uparrow}}$ & & (b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$\\ \cline{1-6}\cline{8-14}

\rule{0pt}{10pt}(c) & $\times$ &  \checkmark & 67.1~$\green{\pmb{\uparrow}}$ & 87.5~$\green{\pmb{\uparrow}}$ & 56.8~$\green{\pmb{\uparrow}}$ & & 
(c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \cline{1-6}\cline{8-14}

\rule{0pt}{10pt}(d) & \checkmark & \checkmark & 66.6~$\green{\pmb{\uparrow}}$ & 87.2~$\green{\pmb{\uparrow}}$ & 57.4~$\green{\pmb{\uparrow}}$  & &
(d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$\\ 
\end{tabular}


% \begin{tabular}{c|c|c|l l l l}

%     & +HIC & +CGLC & Res2 & Res3 & Res4 & Res5 \\ \shline
% (a) & $\times$    & $\times$    & 47.1 & 58.2 & 70.9 & 82.1 \\ \shline
% (b) & \checkmark    & $\times$    & 50.9~$\green{\pmb{\uparrow}}$ & 67.1~$\green{\pmb{\uparrow}}$ & 78.7~$\green{\pmb{\uparrow}}$ & 81.8~$\red{\pmb{\downarrow}}$ \\ \hline
% (c) & $\times$  & \checkmark    & 47.8~$\green{\pmb{\uparrow}}$ & 59.8~$\green{\pmb{\uparrow}}$ & 75.0~$\green{\pmb{\uparrow}}$ & 84.6~$\green{\pmb{\uparrow}}$ \\ \hline
% (d) & \checkmark    & \checkmark    & 51.6~$\green{\pmb{\uparrow}}$ & 69.7~$\green{\pmb{\uparrow}}$ & 82.5~$\green{\pmb{\uparrow}}$ & 84.3~$\green{\pmb{\uparrow}}$ \\ 
% \end{tabular}
% }
% \caption{}
% \label{tab:ab2_new}
% \vspace{-5mm}
% \end{table}

==> tables/algorithm1.tex <==

%##################################################################################################
\begin{algorithm}[t]
\caption{Pseudocode of Intermediate Contrastive Loss.}
\label{alg:detco}
\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{2-5}: 4 different stages of backone, termed res2, res3, res4, res5.
%\vspace{-1.em}
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}

\begin{lstlisting}[language=python]
# net_q: encoder for query
# net_q = {backbone_q, head_q_list=[head 2-5]},  

# net_k: same structure as net_q, encoder  for key
# queue_list: a list of queues 2-5 of K keys (CxK)
# m: momentum
# t: temperature
# x: input image
# w: loss weight for 2-5
# loss_nce: contrastive loss

net_q.params = net_k.params  # initialize
x_q = aug(x)  # a randomly augmented version
x_k = aug(x)  # another randomly augmented version

list_q = backbone_q.forward(x_q)  # list of queries
list_k = backbone_k.forward(x_k)  # list of keys

total_loss = 0 # weight-sum of loss from 4 stages
for i in range(4): # loop through 4 stages
    # feature, queue and weight of current stage
    q = list_q[i] # queries: NxC
    k = list_k[i] # keys: NxC
    queue = queue_list[i] # dictionary of K keys (CxK)
    weight = w[i]
    
    # forward mlp head
    q = head_q_list[i].forward(q)
    k = head_k_list[i].forward(k).detach()
    
    # calculate loss
    loss = loss_nce(q, k, queue, t)
    total_loss = total_loss+loss*weight
    
    # update the queue
    dequeue_and_enqueue(queue, k) 

# SGD update: query network
total_loss.backward()
update(net_q.params)

# momentum update: key network
net_k.params = m*net_k.params+(1-m)*net_q.params


\end{lstlisting}
\end{algorithm}
%##################################################################################################

==> tables/table_c4_fpn_180k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|l l l |l l l |l l l}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-C4 COCO 180k} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 180k} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &35.6           &54.6           &38.2           &31.4           &51.5           &33.5           &36.7           &56.7           &40.0           &33.7           &53.8           &35.9 \\
Supervised   &40.0           &59.9           &43.1           &34.7           &56.5           &36.9           &40.6           &61.3           &44.4           &36.8           &58.1           &39.5 \\ \hline
MoCo\cite{moco}      &40.7\gbf{+0.7} &60.5\gbf{+0.6} &44.1\gbf{+1.0} &35.4\gbf{+0.7} &57.3\gbf{+0.8} &37.6\gbf{+0.7} &40.8\gbf{+0.2} &61.6\gbf{+0.3} &44.7\gbf{+0.3} &36.9\gbf{+0.1} &58.4\gbf{+0.3} &39.7\gbf{+0.2} \\ 
MoCov2\cite{mocov2}      &41.0\gbf{+1.0} &60.6\gbf{+0.7} &44.5\gbf{+1.4} &35.6\gbf{+0.9} &57.2\gbf{+0.7} &38.0\gbf{+1.1} &40.9\gbf{+0.3} &61.5\gbf{+0.2} &44.7\gbf{+0.3} &37.0\gbf{+0.2} &58.7\gbf{+0.6} &39.8\gbf{+0.3} \\ \hline
% DetCo        &\bf{41.4}\gbf{+1.4} &\bf{61.2}\gbf{+1.3} &\bf{44.7}\gbf{+1.6} &\bf{35.8}\gbf{+1.1} &\bf{57.8}\gbf{+1.3} &\bf{38.3}\gbf{+1.4} &\bf{41.5}\gbf{+0.9} &\bf{62.1}\gbf{+0.8} &\bf{45.6}\gbf{+1.2} &\bf{37.6}\gbf{+0.8} &\bf{59.2}\gbf{+1.1} &\bf{40.5}\gbf{+1.0} \\ 
% DetCo+AA     &\bf{41.3}\gbf{+1.3} &\bf{61.2}\gbf{+1.3} &\bf{45.0}\gbf{+1.9} &\bf{35.8}\gbf{+1.1} &\bf{57.9}\gbf{+1.4} &\bf{38.2}\gbf{+1.3} &\bf{41.5}\gbf{+0.9} &\bf{62.5}\gbf{+1.2} &\bf{45.6}\gbf{+1.2} &\bf{37.7}\gbf{+0.9} &\bf{59.5}\gbf{+1.4} &\bf{40.5}\gbf{+1.0} \\ 
DetCo    &\bf{41.3}\gbf{+1.3} &\bf{61.2}\gbf{+1.3} &\bf{45.0}\gbf{+1.9} &\bf{35.8}\gbf{+1.1} &\bf{57.9}\gbf{+1.4} &\bf{38.2}\gbf{+1.3} &\bf{41.5}\gbf{+0.9} &\bf{62.5}\gbf{+1.2} &\bf{45.6}\gbf{+1.2} &\bf{37.7}\gbf{+0.9} &\bf{59.5}\gbf{+1.4} &\bf{40.5}\gbf{+1.0} \\ 

\end{tabular}}
\caption{\textbf{Object detection and instance segmentation fine-tuned on COCO}. 
All methods are pretrained 200 epochs on ImageNet.
DetCo outperforms all supervised and unsupervised counterparts. 
}
\label{tab:coco_180k_c4fpn}
\end{table*}

==> tables/table_c4_fpn_percent1_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|lll|lll|lll}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-FPN COCO 1\% Data} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 2\% Data} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &2.5 &5.8 &1.7 &2.3 &4.9 &1.8 &4.5 &10.3 &3.2 &4.3 &9.3 &3.5 \\
Supervised       &10.0 &19.9 &9.2 &9.7 &18.3 &9.2 &13.7 &26.6 &12.8 &13.0 &24.2 &12.6 \\ \hline
MoCo\cite{moco}             &9.1\rbf{-0.9} &17.3\rbf{-2.6} &8.6\rbf{-0.6} &8.6\rbf{-1.1} &16.1\rbf{-2.2} &8.3\rbf{-0.9} &13.0\rbf{-0.7} &24.1\rbf{-2.5} &12.6\rbf{-0.2} &12.3\rbf{-0.7} &22.4\rbf{-1.8} &12.2\rbf{-0.4} \\
MoCo v2\cite{mocov2}          &9.9\rbf{-0.1}& 18.7\rbf{-1.2} &9.5\gbf{+0.3} &9.5\rbf{-0.2} &17.2\rbf{-1.1} &9.2\rbf{0.0} &13.8\gbf{+0.1} &25.3\rbf{-1.3} &13.4\gbf{+0.6} &12.9\rbf{-0.1} &23.3\rbf{-0.9} &12.7\gbf{+0.1} \\ \hline
% DetCo            &\textbf{10.7}\gbf{+0.7} &\textbf{20.2}\gbf{+0.3} &\textbf{10.4}\gbf{+1.2} &\textbf{10.2}\gbf{+0.5} & \textbf{19.0}\gbf{+0.7} &\textbf{9.9}\gbf{+0.7} &\textbf{14.3}\gbf{+0.6} &\textbf{26.3}\rbf{-0.3} &\textbf{13.9}\gbf{+1.1} &\textbf{13.5}\gbf{+0.5} &\textbf{24.6}\gbf{+0.4} &\textbf{13.1}\gbf{+0.5}\\
% DetCo+AA         &\textbf{12.4}\gbf{+2.4} &\textbf{23.5}\gbf{+3.6} &\textbf{11.8}\gbf{+2.6} &\textbf{12.1}\gbf{+2.4} & \textbf{21.9}\gbf{+3.6} &\textbf{12.0}\gbf{+2.8} &\textbf{16.0}\gbf{+2.3} &\textbf{29.6}\gbf{+3.0} &\textbf{15.6}\gbf{+2.8} &\textbf{15.3}\gbf{+2.3} &\textbf{27.4}\gbf{+2.2} &\textbf{15.1}\gbf{+2.5}\\
DetCo         &\textbf{12.4}\gbf{+2.4} &\textbf{23.5}\gbf{+3.6} &\textbf{11.8}\gbf{+2.6} &\textbf{12.1}\gbf{+2.4} & \textbf{21.9}\gbf{+3.6} &\textbf{12.0}\gbf{+2.8} &\textbf{16.0}\gbf{+2.3} &\textbf{29.6}\gbf{+3.0} &\textbf{15.6}\gbf{+2.8} &\textbf{15.3}\gbf{+2.3} &\textbf{27.4}\gbf{+2.2} &\textbf{15.1}\gbf{+2.5}\\

 

\end{tabular}}
\caption{\small{
\textbf{Semi-Supervised two-stage Detection fine-tuned on COCO 1\% and 2\% data}. All methods are pretrained 200 epochs on ImageNet. \textbf{\green{Green}} means increase and \textbf{\gray{gray}} means decrease. DetCo is better than supervised~/~unsupervised counterparts in all metrics.
}
}

\label{tab:coco_1_2_c4fpn}
\end{table*}

==> tables/table_c4_fpn_percent5_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.75}{
\begin{tabular}{l|lll|lll|lll|lll}
% \hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Mask R-CNN R50-FPN COCO 5\% Data} & \multicolumn{6}{c}{Mask R-CNN R50-FPN COCO 10\% Data} \\ \cline{2-13} 
 & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \shline
\gray{Rand Init} &9.2& 18.6& 7.9& 8.8& 16.9& 8.1 &10.1& 20.2& 9.1& 9.8& 18.6& 9.2 \\
Supervised       &19.9& 37.0& 19.3& 18.6& 33.7& 18.4 &23.8& 42.8& 23.9& 22.2& 39.6& 22.3 \\ \hline
MoCo\cite{moco}             &19.6\rbf{-0.3} &35.1\rbf{-1.9} &20.0\gbf{+0.7} &18.3\rbf{-0.3} &32.3\rbf{-1.4} &18.6\gbf{+0.2} &23.3\rbf{-0.5} &40.7\rbf{-2.1} &23.9\rbf{0.0} &21.9\rbf{-0.3} &38.0\rbf{-1.6} &22.4\gbf{+0.1} \\
MoCo v2\cite{mocov2}          &20.6\gbf{+0.7} &36.6\rbf{-0.4} &21.0\gbf{+1.7} &19.1\gbf{+0.5} &33.7\rbf{0.0} &19.2\gbf{+0.8} &24.1\gbf{+0.3} &42.0\rbf{-0.8} &24.8\gbf{+0.9} &22.5\gbf{+0.3} &39.1\rbf{-0.5} &23.3\gbf{+1.0} \\ \hline
% DetCo            &\textbf{21.4}\gbf{+1.5} &\textbf{38.1}\gbf{+1.1} &\textbf{21.6}\gbf{+2.3} &\textbf{19.9}\gbf{+1.3} &\textbf{35.1}\gbf{+1.4} &\textbf{19.8}\gbf{+1.4} &\textbf{25.3}\gbf{+1.5} &\textbf{43.9}\gbf{+1.1} &\textbf{26.0}\gbf{+2.1} &\textbf{23.6}\gbf{+1.4} &\textbf{40.8}\gbf{+1.2} &\textbf{24.0}\gbf{+1.7} \\
% DetCo+AA        &\textbf{21.9}\gbf{+2.0} &\textbf{39.1}\gbf{+2.1} &\textbf{22.2}\gbf{+2.9} &\textbf{20.4}\gbf{+1.8} &\textbf{36.1}\gbf{+2.4} &\textbf{20.6}\gbf{+2.2} &\textbf{26.0}\gbf{+2.2} &\textbf{45.2}\gbf{+2.4} &\textbf{27.0}\gbf{+3.1} &\textbf{24.3}\gbf{+2.1} &\textbf{42.0}\gbf{+2.4} &\textbf{25.0}\gbf{+2.7} \\
DetCo        &\textbf{21.9}\gbf{+2.0} &\textbf{39.1}\gbf{+2.1} &\textbf{22.2}\gbf{+2.9} &\textbf{20.4}\gbf{+1.8} &\textbf{36.1}\gbf{+2.4} &\textbf{20.6}\gbf{+2.2} &\textbf{26.0}\gbf{+2.2} &\textbf{45.2}\gbf{+2.4} &\textbf{27.0}\gbf{+3.1} &\textbf{24.3}\gbf{+2.1} &\textbf{42.0}\gbf{+2.4} &\textbf{25.0}\gbf{+2.7} \\

\end{tabular}}
\caption{\small{
\textbf{Semi-Supervised two-stage Detection fine-tuned on COCO 5\% and 10\% data}. All methods are pretrained 200 epochs on ImageNet. DetCo is better than supervised~/~unsupervised counterparts in all metrics.
}
}

\label{tab:coco_5_10_c4fpn}
\end{table*}

==> tables/table_lvis.tex <==
\begin{table}[]
\centering
\scalebox{0.90}{
\begin{tabular}{l|ccc|ccc}
Method     & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$ & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ \\ \hline
\gray{Rand Init}  & 19.6 & 31.8   & 20.9   & 19.0 & 29.8   & 20.1   \\ 
Supervised & 22.7 & 36.8   & 24.1   & 22.2 & 34.6   & 23.5   \\ \hline
MoCo\cite{moco}   & 23.1 & 37.4   & 24.5   & 22.5 & 35.1   & 23.8   \\ 
MoCo v2\cite{mocov2}    & 23.2 & 37.4   & 24.7   & 22.8 & 35.1   & 24.4   \\ \hline
DetCo      & \bf{23.5} & \bf{37.7}   & \bf{24.8}   & \bf{23.0} & \bf{35.5}   & \bf{24.5}   \\ 
\end{tabular}}
\caption{\textbf{DetCo \textit{vs.} supervised and other unsupervised methods on LVIS v1.0 dataset.} 
All methods are pretrained 200 epochs on ImageNet.
We evaluate object detection and instance segmentation tasks.}
\label{tab:lvis}
\vspace{-5mm}
\end{table}
